Multi hash embeddings in spaCy

The distributed representation of symbols is one of the key technologies in machine learning systems today, playing a pivotal role in modern natural language processing. Traditional word embeddings associate a separate vector with each word. While this approach is simple and leads to good performance, it requires a lot of memory for representing a large vocabulary. To reduce the memory footprint, the default embedding layer in spaCy is a hash embeddings layer. It is a stochastic approximation of traditional embeddings that provides unique vectors for a large number of words without explicitly storing a separate vector for each of them. To be able to compute meaningful representations for both known and unknown words, hash embeddings represent each word as a summary of the normalized word form, subword information and word shape. Together, these features produce a multi-embedding of a word. In this technical report we lay out a bit of history and introduce the embedding methods in spaCy in detail. Second, we critically evaluate the hash embedding architecture with multi-embeddings on Named Entity Recognition datasets from a variety of domains and languages. The experiments validate most key design choices behind spaCy's embedders, but we also uncover a few surprising results.

==> extras/history_rant.tex <==
These tokens themselves do not have
any particular information embedded in their surface forms i.e.: from the orthographic
rendition of the word ``w i z a r d'' it is not clear what the word means. Furthermore, consider
the widespread phenomenon across languages called \emph{homophony},
where multiple quite distinct meanings are indexed by the same word form. 
In English for example the words ``sole'' and ``soul'' are written differently, but are pronounced the same.
Hungarian has a writing system that follows pronunciation more closely and the words
``throw'' and ``drum'' can be translated to the word written as ``dob''.

The theory that forms are unrelated to meaning in linguistics
is often expressed as \emph{the arbitrariness of the sign} and dates back all the way
to the beginnings of structuralism and the birth of semiotics \cite{de1916nature}. 
There is some evidence against complete arbitrariness, however, the consensus
is that even if there are systematic form-meaning associations, 
they are very weak \cite{pimentel2021finding}. Interestingly, the situation in NLP is
in stark contrast with some other areas of machine cognition that are focused on
interpreting physical signals such as computational processing of speech and vision.
In these areas there is an abundance of information presented in the input -- albeit often
noisy and incomplete -- and the task is to extract the relevant structure for the task at hand.

The question for us is then: how can we provide useful prior information to computational
models about lexical units? The currently the popular and successful answer of
pre-training word embeddings was brewed in the early days of connectionism. 
The birth of representing symbols
in neural networks revolves around the notion of computational models of \emph{associative memory}
\citet{kohonen1972correlation,little1974existence,hopfield1982neural}. Associative memory
is an explicit memory that allows for (almost) exact recall of arbitrary
items (more or less) consciously based on relationships between these items. 
The most influential model of associative memory are Hopfield Networks that originate
from the Ising Model which is a square grid of interacting binary cells used in
statistical mechanics. Thinking about models of associative memory in terms of 
models of statistical mechanics has impacted connectionist thinking
to the point that the relationships between modern variants of continuous state
Hopfield Networks and Transformers is fairly transparent \cite{ramsauer2020hopfield}.

Back to our problem, word representations. At the time the question was how is it possible 
to understand such high-level cognition as concept representation and
associative memory recall as a spontaneous emergent behavior of many interacting
simple neurons. In such models of concepts and memory each symbol or unit of ``knowledge''
is represented by a pattern of activations across neurons in a simple simulated model
of human brain \citet{hinton1986learning}. Practically speaking, we represent each input
symbol as a list of numbers, where each number corresponds to a response from an artificial neuron.
This is exactly the idea we use these days to represent words as embeddings. 
We train artificial neural networks and learn word representations that are real valued
vectors.

The big practical advantage of artificial neural networks over many other approaches
to cognitive problems such as machine language processing is that they are designed to ingest
a large variety of inputs and extract statistical regularities from them without many assumptions.

 Often \emph{distributed}
representations are considered analogous to \emph{real-valued} vectors, but earlier
models like the ones based on the Ising model used binary representations. 
However, the popularity of the backpropagation algorithm \citep{linnainmaa1970representation,rumelhart1986learning}
meant moving away from discrete representations that do not admit
gradient based optimization.

==> extras/pretraining.tex <==
\begin{comment}
    
\subsection{Pretraining algorithms}

%The word-embedding learning algorithm we use to train vectors for spaCy is called \texttt{floret} and is based on the \texttt{fastText} algorithm. 
%Many other approaches exist. %, but it has been theoretically discovered
%that m
%Most of them implicitly approximate the pointwise-mutual information (PMI) between words in the corpus.
%In computational linguistics, PMI has been used as an intuitive and successful way of measuring the association between
%words. Its definition is quite intuitive:

%\begin{equation}
%    \text{PMI}(w_i, w_j) = \log_2 \frac{p(w_i, w_j)}{p(w_i) p(w_j)}
%\end{equation}

%When the joint probability of two words equals the product of marginals $p(w_i, w_j) = p(w_i) p(w_j)$
%it means that $p(w_i|w_j) = p(w_i)$ in which case the words are independent and $\text{PMI}(w_i, w_j) = 0$.
%The empirical estimate of the $\text{PMI}(w_i, w_j)$ can be computed using simply counting: the number of words
%in the corpus $N$ the number of times $w_i$ and $w_j$ co-occur $N_{ij}$ and the number of 
%times they occur overall $N_i$, $N_j$: $\frac{N_{ij} \times N}{N_i \times N_j}$. We can think
%of PMI as a matrix where $\text{PMI}_{ij}$ is the entry $\text{PMI}(w_i, w_j)$. Point-wise
%mutual information has been used in a wide range of NLP applications for example
%identifying idiomatic expressions \citep{fazly2009unsupervised}, 
%online review classification \citet{turney2002thumbs},  phrase mining for social media analysis
%\citet{schwartz2013personality} and grounding the word-meanings in the visual world \citet{young2014image}.

%The embedding algorithms learn two embeddings tables: one for the words representations 
%$\mathbf{E}_w \in \mathbb{R}^{n \times d}$ used in downstream tasks and 
%another for context representations $\mathbf{E}_c \in \mathbb{R}^{m \times d}$ used only for training.
%It can be shown theoretically that many embedding algorithms learn embedding matrices where the inner
%product between the word- and context-vectors $\mathbf{w}_i^T\mathbf{c}_j$ approximates a quantity
%related to pointwise-mutual information (PMI) between the two words \citep{kenyon2020deconstructing}. The is an intuitive and successful way of measuring the association between words that has been used
%before for identifying idiomatic expressions \citep{fazly2009unsupervised}, 
%online review classification \citet{turney2002thumbs},  phrase mining for social media analysis
%\citet{schwartz2013personality} and grounding the word-meanings in the visual world \citet{young2014image}. Word-embedding algorithms
%learn a low-rank factorization that is related to PMI: $\mathbf{E}_c \mathbf{E}_w^T \approx \phi(\text{PMI})$, 
%where $\phi(\text{PMI})$ is some simple function of the $\text{PMI}$ matrix and both $\mathbf{E}_w$ and $\mathbf{E}_c$ are lower rank than $\text{PMI}$ since $\text{PMI} \in \mathbb{R}^{n \times m}$, $\mathbf{E}_w \in \mathbb{R}^{n \times d}$,
%$\mathbf{E}_c \in \mathbb{R}^{m \times d}$ and $n \gg d$ and $m \gg d$. 


The learning algorithm we used to train word embeddings for spaCy is called floret, and it is based on the 
fastText algorithm. The fastText package implements two algorithms
from the seminal word2vec package called skip-gram and CBOW (continuous bag-of-words).
The models were trained to maximize the likelihood of a corpus with words $w_1, \ldots, w_t \in D$, where the number of words in the corpus $|D|$ is in the billions. They learn the word embeddings $\mathbf{w} \in \mathbb{R}^d$ and context embeddings $\mathbf{w} \in \mathbb{R}^d$ the same size $d$ for each word. It is well known that the skip-gram embeddings trained with the negative sampling 
algorithm learn embeddings that approximate the pointwise mutual information between words which is a commonly used measure of association between words: $\mathbf{w}^T\mathbf{c} \approx \text{PMI}(w, c) - 
\log k$, where $k$ is the constant hyperparameter of the algorithm defining the number of negative 
samples per update as presented in the seminal paper \citep{levy2014neural}. 

% But why not just explicitly factorize the PMI matrix? 
% In their follow-up work they do show that applying Singular-Value Decomposition (SVD) to an empirical PMI matrix
% works just as well as other word-embedding learning algorithms \citep{levy2015improving}. 
% However, \emph{explicitly} storing the PMI matrix and running full SVD on it makes the 
% algorithm scale poorly as the vocabulary size increases.

\subsubsection{Training}

Even though the \emph{implicit} objective of the algorithms in fastText revolves around the 
PMI between words the \emph{concrete} implementation looks deceptively different. 
The objective of the algorithm is inspired by trying to maximize the likelihood of the corpora,
but through efficient factorizations and approximations. 
There are many different ways of breaking down the likelihood of a sequence of words 
$p(w_1, \ldots, w_t)$ into smaller more manageable factors. Using the notation $w_{n:1}$
meaning the ``the sequence of words from 1 to $n$'' for example we can write the probability of the full sequence as:

\begin{equation*}
    p(w_{1:n}) = p(w_1)p(w_2|w_1)p(w_3|w_1; w_2) \ldots p(w_n|w_{1:n-1}) = \prod_{i=1} p(w_i|w_{1:i-1}) 
\end{equation*}

This autoregressive factorization is has been around since the 1980s \citep{jelinek1980interpolated}
and is still underlying some of the most popular modern language models such as the GPT family \citep{radford2019language}
from OpenAI. When learning word representations $\mathbf{E}_w$, however, we are not really
interested in accurately capturing $p(w_1, \ldots, w_n)$, because we have no intention to
generate from this distribution or evaluate the likelihood of sequences under our model. 
What we are looking is a factorization that is really
cheap to compute over huge datasets and leads to useful representations. The \texttt{skipgram} algorithm
picks a small context size $c$ (usually around 4) and computes the likelihood of the sequence 
$w_1, \ldots, w_n$ as 

\begin{equation*}
    p(w_1, \ldots, w_n) = \prod_{i=1}^n \prod_{-c \leq j \leq c, j \neq 0} p(w_{i+j}|w_i)
\end{equation*}

There is a dedicated focus word $w_i$, and we pick words around it $w_{i+j}$, both left and right,
up to context size $c$. When optimizing the (log)-likelihood with the skipgram factorization
the word representations are trained to be predictive of their environment. 
One way to compute each single factor $p(w_{i+j}|w_i)$ is to use the \texttt{softmax}
function. We pick the representation $\mathbf{w}$ of the context word $w$ from the embedding table
 $\mathbf{E}_w$, and the context representation $\mathbf{c}$ for the word $w_{i+j}$ from $\mathbf{E}_c$. Now we can write

 \begin{equation}
    p(w_{i+j}|w_i) = \frac{\exp(\mathbf{w}^T\mathbf{c})}{\sum_{i=1}^{|\Sigma|}  \exp(\mathbf{w}^T\mathbf{c}_i)}
 \end{equation}

The summation in the denominator is  expensive to evaluate if we want to train a large vocabulary $|\Sigma|$. 
Instead of the full
softmax, we can instead just distinguish between ``good'' and ``bad'' pairs of words. The noise-contrastive estimation
framework replaces this multi-class classification problem with a series of binary classification 
problems. This eliminates the expensive normalization term (the sum). Using the notation $\sigma(x)$ for the logistic
function, the objective that the skipgram model with $k$ negative samples is trying to minimize is:

\begin{equation}
    -\sum_{w_i, w_j \in D} \left[ \log \sigma(\mathbf{w}_i^T\mathbf{c_j}) + \sum_{\ell = 1}^k \mathbb{E} \left[\log (1 - \sigma(\mathbf{w}_i^T \mathbf{c_\ell})  \right] \right]
\end{equation}

Here $\log \sigma(\mathbf{w}_i^T\mathbf{c_j})$ is the log-likelihood that a word pair $w_i, w_j$ comes from the 
actual corpus. Then $\log (1 - \sigma(\mathbf{w}_i^T \mathbf{c_\ell}))$ corresponds to the log-likelihood that
a fake word pair $w_i, w_\ell$ did not come from a noise distribution: We draw $k$ distractor words $c_\ell$
according to a smoothed unigram distribution. This objective leads to a practical and very successful algorithm
that only requires sampling real- and fake-pairs over a large corpus and computing the above objective. The
\texttt{cbow} algorithm is very similar, but rather than predicting context from focus words it predicts focus
words from context using a pooling over context words.

\subsubsection{Subwords}

The fastText \citep{bojanowski2016enriching} algorithm adds a small, but empirically very useful modification to the \texttt{word2vec}
algorithms: multi-embeddings. Rather than representing words as atomic, it uses the sum of character $n$-grams
as the representation of each word during training. %[extend a bit]

%The \texttt{fastText} implementation stores two vector tables: one for the 
%words and one for subwords. 

% The \texttt{floret} algorithm in spaCy marries \texttt{fastText} and Bloom embeddings.
%Only one embedding table is stored in \texttt{floret} shared between words and subwords and each word or subword
%is hashed multiple times using the Bloom embedding trick. This allows \texttt{floret} to store (an order of 
%magnitude) fewer word vectors -- going from millions to hundreds of thousands -- resulting in a dramatic reduction
%in space, from around 3GB down to less than 300MB in practice.
\end{comment}
